Improved Local Computation Algorithm for Set Cover via Sparsification

We design a Local Computation Algorithm (LCA) for the set cover problem. Given a set system where each set has size at most $s$ and each element is contained in at most $t$ sets, the algorithm reports whether a given set is in some fixed set cover whose expected size is $O(\log{s})$ times the minimum fractional set cover value. Our algorithm requires $s^{O(\log{s})} t^{O(\log{s} \cdot (\log \log{s} + \log \log{t}))}$ queries. This result improves upon the application of the reduction of [Parnas and Ron, TCS'07] on the result of [Kuhn et al., SODA'06], which leads to a query complexity of $(st)^{O(\log{s} \cdot \log{t})}$. To obtain this result, we design a parallel set cover algorithm that admits an efficient simulation in the LCA model by using a sparsification technique introduced in [Ghaffari and Uitto, SODA'19] for the maximal independent set problem. The parallel algorithm adds a random subset of the sets to the solution in a style similar to the PRAM algorithm of [Berger et al., FOCS'89]. However, our algorithm differs in the way that it never revokes its decisions, which results in a fewer number of adaptive rounds. This requires a novel approximation analysis which might be of independent interest.

==> alg-sparsify-stages.tex <==


\subsection{Sparsification of the Outer Loop}

\begin{algorithm}
	\caption{\label{alg:main-alg-sparsify-stages}}
	
	Let $(\cS,\cE)$ be some set cover instance.
	
	\For{each pair of $(i,l)$ where $i \in [\log s]$ and $l \in [\log t]$}{		
		$B_i(S)$ and $\cS_{i,l}$ are generated in the exact same way as in \cref{alg:generic-alg}	
	}
	
	\For{stage i = 1 to $\log s$}{	
		Let $\cE_i$ be the set of uncovered elements
		
		
		\For{each set $S \in \cS$}{
			
			$\hat{B}_i(S) \gets B_i(S) \cap \cE_i$	
			
			\If{$|\hat{B}_i(S)| \geq \logten$}{
				\tcp{only happens if $S$ is a "bad" set} 
				{\bf add} $S$ to the set cover.  		
			}
		}
		
		
		\For{each $l \in [\log (t)]$}{		 		
			$\hcS_{i,l} \gets \{S|S \in S_{i,l}, \degree(S) \geq s/2^i\}$ 			
			\For{each $e \in \cE_i$ in parallel}{

				\If{the degree of $e$ in $\hcS_{i,l}$ is more than $\logten \cdot 2^l$}{ \label{line:sparse-main-if-high-degree-element}}{
					\tcp{only happens if $e$ is a "bad" element.}

				\If{the degree of $e$ in $\hcS_{i,l}$ is more than $\logten \cdot 2^l$}{ \label{line:loglog-if-high-degree-element}}{
					\tcp{only happens if $e$ is a "bad" element; $e$ will be covered in \cref{line:sqrt-t-clean-up}.}

					
					\label{line:sparse-main-pretend-1}
					{\it pretend that $e$ is covered.} 
				}
			}

		}		 	
	For each uncovered element $e$, add some arbitrary set which contains $e$ to the set cover
}
\end{algorithm}
\begin{algorithm}
	\caption{$\RecSplit(i', R, i, \hat{B}_{[i',i'+R-1]} = (\hat{B}_{i'}, \hat{B}_{i'+1},...,\hat{B}_{k'+R - 1}), \hcE_i)$\label{alg:rec-sparse}}
	\KwIn{\\
		\quad Simulates iterations $k'$ to $k'+R-1$ of the $i$-th iteration  \\
		\quad For $k \in \{k',...,k'+R-1\}$, $\hcS_k$ consists of sets that will be added to the set cover as long as the estimated number of free elements is at least $s/2^i$ in the beginning of the $k$-th iteration of stage $i$. \\
		\quad $\hat{\cE}_i$ consists of all elements which are uncovered (and don't pretend to be covered) at the beginning of iteration $k'$
	} 
	
	\If{$R \le \log \log{t}$}{
		$BaseCase(k', R, i, (\hcS_{k'},\hcS_{k'+1},...,\hcS_{k'+R-1}), \hcE_i)$ \\
		return
	}		
	
	
	$\RecSplit(k', R/2, i, (\hcS_{k'},\hcS_{k'+1},...,\hcS_{k'+R/2 - 1}), \hcE_i)$ \label{line:sparse-1st-rec-call}
	
	
	
	\For{each $k \in \{k'+R/2,...,k'+R-1\}$}{		 
		
		$\cS'_{k} \gets \{S|S \in \hcS_{k}, \degree(S) \geq s/2^i\}$ 
		
		\For{each uncovered element $e$ in parallel}{
			\If{the degree of $e$ in $\cS'_k$ is more than $\logten \cdot 2^{k-(k' + R/2)}$}{ \label{line:loglog-if-high-degree-element-2}}{
				\tcp{only happens if $e$ is a "bad" element}
				
				\label{line:alg-3-pretend-2}
				{\it pretend that $e$ is covered.} 
			}
		}
	}	
	
	$\cE'_i \gets $ all uncovered elements in $\hat{\cE}_i$ 
	
	$\RecSplit(k'+R/2, R/2, i, (\cS'_{k'+R/2},\cS'_{k'+R/2+1},...,\cS'_{k'+R-1}), \cE'_i)$ \label{line:2nd-rec-call}
\end{algorithm}

\begin{algorithm}
	\caption{$BaseCase(i', R, \hat{B}_{[i',i'+R-1]} = (\hat{B}_{i'}, \hat{B}_{i'+1},...,\hat{B}_{i'+R - 1}), \hcE_i)$\label{alg:base_case-sparse}}
	
	\For{stage $i = i'$ to $i' + R - 1$}{
		
		\RecSplit()
	}		

		}
	}

\end{algorithm}

==> tmp.tex <==
\section{An attempt to make \cref{alg:rec-split} sequential}

\begin{algorithm}
	$T \eqdef \sqrt{\log(t)}$
	
	\For{stage $i = 1$ to $\log s$}{
		Let $\cE_i$ be the set of elements not covered so far.
		
		$\cS_i \gets $ all the sets $S$ such that $S$ is not in the cover and $|S \cap \cE_{i, j}| \ge s / 2^i$. 
	
		For $k \in \{1,...,T\}$ and $j \in \{0, \ldots, T - 1\}$, let $\cS_{i,j,k}$ be a subset of $\cS_i$ where each $S \in \cS_i$ is included independently to $\cS_{i, j, k}$ with a probability of 
		$p_k$ where  $p_k = \frac{2^{j \cdot T + k}}{t}$. 
					 
		\For{phase $j = 0$ to  $T-1$}{
			\For{iteration k = 1 to $T$ }{
				\For{each set $S \in \cS_{i,j,k}$ in parallel} {
		    	Let $\hat{d}_{i,j,k}(S)$ be an estimate of the total number of free elements in $S$. This estimate is obtained by sampling a fresh batch of $\log t \cdot \log^5 s$ elements in $S \cap \cE_{i, j}$ and checking how many of them are free. 
					
		    	\If{$\hat{d}_{i,j',k'}(S) \geq s/2^i$ for all iterations $(i,j',k')$ up to and including $(i,j,k)$}{
		    	Add $S$ to the set cover 
	    	}

				}
			\For{each free element $e$ in parallel } {
				\If{the degree of $e$ in $\cS_{i, j, k}$ is more than $4 \cdot \log^2 s \cdot 2^{3T}$ }{
					Mark $e$ as heavy and in the future consider as covered.
				}
			}

			} 
		}
		
		\For{each element $e$ that got heavy in this stage} {
			Cover $e$ by the set with the smallest ID among all containing $e$.
		}
		
		\For{each set $S$ in parallel } {
			Add to the cover $S$ if the number of free elements in $S$ is more than $s / 2^i$. 
		}
	}
	\caption{A simulation in LCA that requires $(st)^{O(\log{s} \sqrt{\log{t}})}$ many queries.}
\end{algorithm}

